Adaptive Malware Detection using Sequential Feature Selection: A Dueling Double Deep Q-Network (D3QN) Framework for Intelligent Classification

Traditional malware detection methods exhibit computational inefficiency due to exhaustive feature extraction requirements, creating accuracy-efficiency trade-offs that limit real-time deployment. We formulate malware classification as a Markov Decision Process with episodic feature acquisition and propose a Dueling Double Deep Q-Network (D3QN) framework for adaptive sequential feature selection. The agent learns to dynamically select informative features per sample before terminating with classification decisions, optimizing both detection accuracy and computational cost through reinforcement learning. We evaluate our approach on Microsoft Big2015 (9-class, 1,795 features) and BODMAS (binary, 2,381 features) datasets. D3QN achieves 99.22% and 98.83% accuracy while utilizing only 61 and 56 features on average, representing 96.6% and 97.6% dimensionality reduction. This yields computational efficiency improvements of 30.1x and 42.5x over traditional ensemble methods. Comprehensive ablation studies demonstrate consistent superiority over Random Forest, XGBoost, and static feature selection approaches. Quantitative analysis demonstrates that D3QN learns non-random feature selection policies with 62.5% deviation from uniform baseline distributions. The learned policies exhibit structured hierarchical preferences, utilizing high-level metadata features for initial assessment while selectively incorporating detailed behavioral features based on classification uncertainty. Feature specialization analysis reveals 57.7% of examined features demonstrate significant class-specific discrimination patterns. Our results validate reinforcement learning-based sequential feature selection for malware classification, achieving superior accuracy with substantial computational reduction through learned adaptive policies.

==> section_4_Implementation_and_algorithm.tex <==
All the tests and experiments conducted in this research were executed using a Desktop machine with 32GB RAM and NVIDIA GeForce RTX $3070$ graphic card. For the implementation of the classification policy network, a PyTorch framework was implemented. 

We evaluate our proposed algorithm for two benchmark datasets, that are, Microsoft malware challenge (BIG 2015) and Blue Hexagon Open Dataset for Malware AnalysiS (BODMAS) datasets, (Details shown in Figure ~\ref{fig:Samples} and ~\ref{fig:BODMAS} in Supplementary), comprised by different numbers of malware families \cite{ronen2018microsoft}\cite{bodmas}. Different statistical and structural features sets from both the datasets are used to train and evaluate the performance of the proposed algorithm. For BIG 2015 dataset, We used the features defined in \cite{ahmadi2016novel}, that are, feature sets defining the hexadecimal description towards the binary contents of the file and assembly view of various metadata information, for instance, strings, function call, etc., obtained as of the binary using IDA disassembler tool. For BODMAS dataset, we used the defined pre-extracted features by \cite{bodmas}, which follows the same feature format of EMBER \cite{2018arXiv180404637A} and SOREL-20M \cite{harang2020sorel}, consisting eight groups of raw features that include five groups of parsed features generated through Portable Executable (PE) file parser and three groups are format-agnostic feature set which do not require parsing of the PE file during extraction. \par

%We use Dueling Double Deep Q-Network (D3QN) as a policy network (agent) to build an optimal classification policy network $Q^*$ consisting of an input layer to accept the sample’s state, three fully connected hidden layers with PReLU activation, and the output Q-values for each possible action in the recently observed state is aggregated from the two estimators generated from the last layer of the network, i.e., one function estimating value of the current state and other function estimating advantage of taking a specific action in that state. The aggregation of the output of these two estimators accelerate the agent to focus more on the advantageous action (Equation. \textbf{\ref{eq_8}}). As stated earlier, this new neural network design is better suited for model-free reinforcement learning problems and results to accelerate and stabilize the training process unlike other approximating networks. \par

%According to the defined MDP environment, the training of the agent is carried out as an episodic task, where every single episode relates to a sample (x, y) from the training dataset, drawn randomly. We build upon prior work \cite{janisch2019classification}, that defines the observed state of the selected sample in the form of $s={(x^{(i)}, f_i)| \forall f_i \in F}$, explained in section III.  Here the state of the malware executable sample can be defined as the selected features from the original sample by the environment. Shown above the episodic classification task of our policy network in figure \textbf{\ref{fig:Decision-making-system}}, in which the initial state discloses no information about the selected sample's class, showing the scenario of starting investigation about an unknown file where the policy network, i.e., agent, will try to get information about the given file using feature selection actions ($a = A_f $) incrementally. The agent, with the goal of revealing minimum information-rich features, terminate the episode after getting enough information about the selected sample by executing a final classification decision action ($a = A_c $). \par 

To overcome the correlation effect occurring in the policy network's parameters and to make the learning more generalised, the training of the network has been done using Experience Replay-memory where multiple episodic experiences of the environment are stored and each experience represents a specific state record of a malware sample along with the corresponding action ($ a = A_f / A_c $) value, plus reward $r$ and next state $s'$ of the sample. These episodes are stored as a copy of the original file, which reveals different features of the original file. To optimize the policy network, a batch of experiences is tested randomly from the replay buffer and their normalized gradient is backpropagated. The whole RL agent learning architecture can be seen in Figure \textbf{\ref{fig:D3QN_Model_archetecture}}. The training of the policy network on these previous experiences will try to develop a classification policy, which will make an accurate prediction about the class of the sample after revealing a minimum number of features from the input coming file.

%This learning methodology enhance the decision process with the intuition of speeding the malware detection and classification process by selecting only the information-rich features for the given test sample. 


\begin{figure}[htp]
\includegraphics[width=\linewidth]{Evl_Training.png}
\centering
        \caption{Average Episode Length and Average Accuracy measured on the validation dataset during training for both DDQN and D3QN. These plots illustrate the learning dynamics of the two multi-class classification policy networks trained on the Big2015 dataset using a reduced feature set comprising \textbf{1795} features. From the figures, it is evident that our proposed D3QN architecture demonstrates improved performance, achieving higher accuracy with shorter episode lengths. The reduced episode length corresponds to fewer penalties incurred, indicating more efficient decision-making over time.}
    \label{fig:Training_evl}
\end{figure}
